A low-PAPR Pilot Design and Optimization for OTFS Modulation

Orthogonal time frequency space (OTFS) modulation has been proposed recently as a new waveform in the context of doubly-selective multi-path channels. This article proposes a novel pilot design that improves OTFS spectral efficiency (SE) while reducing its peak-to-average power ratio (PAPR). Instead of adopting an embedded data-orthogonal pilot for channel estimation, our scheme relies on Chu sequences superimposed to data symbols. We optimize the construction by investigating the best energy split between pilot and data symbols. Two equalizers, and an iterative channel estimation and equalization procedure are considered. We present extensive numerical results of relevant performance metrics, including the normalized mean squared error of the estimator, bit error rate, PAPR and SE. Our results show that, while the embedded pilot scheme estimates the channel more accurately, our approach yields a better tradeoff by achieving much higher spectral efficiency and lower PAPR.

==> tex/notation.tex <==
%%%% Environments

\newtheorem{definition}{Definition}
\newtheorem{observation}{Observation}

\DeclareRobustCommand{\emphbox}[1]{%
\begin{tcolorbox}[ 
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=gray!15,
        colframe=black,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=6pt,
        arc=2pt,outer arc=2pt,
        boxrule=0.3pt,
        fontupper=\itshape,
        ]
        #1
\end{tcolorbox}
}

\newcommand{\boxtitle}[1]{{\normalfont \textbf{\textsf{#1}}}}
\newcommand{\asmp}[1]{{\normalfont\small \textsf{[A#1]}}}

%%%% Framing

\newcommand{\NS}{\mathtt{N}_{\scaleto{\mathsf{S}}{3.5pt}}}
\newcommand{\NC}{\mathtt{N}_{\scaleto{\mathsf{C}}{3.5pt}}}
\newcommand{\NFFT}{\mathtt{N}_{\scaleto{\mathsf{FFT}}{3.5pt}}}

\newcommand{\numer}{\mu}

\newcommand{\pilot}{\bm{x}_{\scaleto{\mathsf{P}}{3.5pt}}}
\newcommand{\pilotobs}{\bm{y}_{\scaleto{\mathsf{P}}{3.5pt}}}

\newcommand{\preamblelength}{n_{\scaleto{\mathsf{PRE}}{3.5pt}}}
\newcommand{\POlength}{n_{\scaleto{\mathsf{PO}}{3.5pt}}}

%%%%% UMAC
\newcommand{\PUPE}{\mathsf{PUPE}}
\newcommand{\inalpha}{\mathcal{X}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\code}{\mathcal{C}}


%%%%% Wireless
\newcommand{\NRX}{N_{\scaleto{\mathsf{RX}}{3.5pt}}}



%%%%%% Math
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
